Gradient Deconfliction via Orthogonal Projections onto Subspaces For Multi-task Learning

Although multi-task learning (MTL) has been a preferred approach and successfully applied in many real-world scenarios, MTL models are not guaranteed to outperform single-task models on all tasks mainly due to the negative effects of conflicting gradients among the tasks. In this paper, we fully examine the influence of conflicting gradients and further emphasize the importance and advantages of achieving non-conflicting gradients which allows simple but effective trade-off strategies among the tasks with stable performance. Based on our findings, we propose the Gradient Deconfliction via Orthogonal Projections onto Subspaces (GradOPS) spanned by other task-specific gradients. Our method not only solves all conflicts among the tasks, but can also effectively search for diverse solutions towards different trade-off preferences among the tasks. Theoretical analysis on convergence is provided, and performance of our algorithm is fully testified on multiple benchmarks in various domains. Results demonstrate that our method can effectively find multiple state-of-the-art solutions with different trade-off strategies among the tasks on multiple datasets.

==> tex/frontinfo.tex <==
%%
%% The "title" command has an optional parameter,
%% allowing the author to define a "short title" to be used in page headers.
% \title{The Name of the Title is Hope}

\title{Gradient Deconfliction via Orthogonal Projections onto Subspaces For Multi-task Learning}

%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.
% \author{Brooke Aster, David Mehldau}
% \email{dave,judy,steve@university.edu}
% \email{firstname.lastname@phillips.org}


% \setcopyright{acmcopyright}
% \copyrightyear{2018}
% \acmYear{2018}
% \acmDOI{10.1145/1122445.1122456}

% %% These commands are for a PROCEEDINGS abstract or paper.
% \acmConference[Woodstock '18]{Woodstock '18: ACM Symposium on Neural
%   Gaze Detection}{June 03--05, 2018}{Woodstock, NY}
% \acmBooktitle{Woodstock '18: ACM Symposium on Neural Gaze Detection,
%   June 03--05, 2018, Woodstock, NY}
% \acmPrice{15.00}
% \acmISBN{978-1-4503-XXXX-X/18/06}

% \author{Shijie Zhu}
% \authornote{both authors contributed equally to this research.}
% \affiliation{%
%   \institution{Alibaba Group}
%   \city{Hangzhou}
%   \country{China}
% }
% \email{shuyuan.cy@alibaba-inc.com}

% \author{Hui Zhao}
% \affiliation{%
%   \institution{Alibaba Group}
%   \city{Hangzhou}
%   \country{China}}
% \email{shuqian.zh@alibaba-inc.com}

% \author{Pengjie Wang}
% \affiliation{%
%   \institution{Alibaba Group}
%   \city{Hangzhou}
%   \country{China}}
% \email{pengjie.wpj@alibaba-inc.com}

% \author{Jian Xu}
% \affiliation{%
%   \institution{Alibaba Group}
%   \city{Hangzhou}
%   \country{China}}
% \email{xiyu.xj@alibaba-inc.com}

% \author{Bo Zheng}
% \authornote{Corresponding author: Bo Zheng.}
% \affiliation{%
%   \institution{Alibaba Group}
%   \city{Hangzhou}
%   \country{China}}
% \email{bozheng@alibaba-inc.com}




%%
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.
% - \renewcommand{\shortauthors}{Yu Chen, et al.}

% \shortauthors{AA,BB,CC}
%%


%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%

% \ccsdesc[500]{Information systems~Computational advertising}

% \ccsdesc[500]{Computer systems organization~Embedded systems}
% \ccsdesc[300]{Computer systems organization~Redundancy}
% \ccsdesc{Computer systems organization~Robotics}
% \ccsdesc[100]{Networks~Network reliability}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
%\keywords{Delayed Feedback, Online Adevertising, CVR prediction}

%% A "teaser" image appears between the author and affiliation
%% information and the body of the document, and typically spans the
%% page.
% \begin{teaserfigure}
%   \includegraphics[width=\textwidth]{sampleteaser}
%   \caption{Seattle Mariners at Spring Training, 2010.}
%   \Description{Enjoying the baseball game from the third-base
%   seats. Ichiro Suzuki preparing to bat.}
%   \label{fig:teaser}
% \end{teaserfigure}

%%
%% This command processes the author and affiliation and title
%% information and builds the first part of the formatted document.

==> tex/prelim_backup.tex <==


\paragraph{Problem Definition.}
For multi-task learning(MTL) problems with $T > 1$ tasks, a collection of $N$ data points $\{\textbf{x}_i,\textbf{y}_i\}$, where $\textbf{y}_i=(y_i^1,...,y_i^T)$ with $y_i^t$ as the label of task $\mathcal{T}_t$, are $i.i.d.$ sampled from input feature space $\mathcal{X}$ and task spaces $\{\mathcal{Y}^t\}_{t\in\{1,..,T\}}$. 
A multi-task model is usually designed as $f^t(\mathbf{x};\boldsymbol{\theta}^{sh},\boldsymbol{\theta}^{t}): \mathcal{X}\longrightarrow \mathcal{Y}^t$ for each task with shared structures determined by parameters $\boldsymbol{\theta}^{sh}$ across all tasks and task-specific parts by $\boldsymbol{\theta}^{t}$. The task-specific differentiable loss functions $\mathcal{L}_t(\boldsymbol{\theta}^{sh},\boldsymbol{\theta}^{t}):\mathcal{Y}^t\times\mathcal{Y}^t\longrightarrow \mathbb{R}^+$ are empirically defined as $\hat{\mathcal{L}}_t(\boldsymbol{\theta}^{sh},\boldsymbol{\theta}^{t}):=\frac1N \sum_i \mathcal{L}_t(f^t(\mathbf{x};\boldsymbol{\theta}^{sh},\boldsymbol{\theta}^{t}), y_i^t)$. In common practice, a standard objective for MTL is to minimize the average loss over all tasks:
\begin{align}
\label{eq:avg_loss}
(\boldsymbol{\theta^{sh}}_{optimal}, \boldsymbol{\theta^{t}}_{optimal})=\argmin_{(\boldsymbol{\theta}^{sh},\boldsymbol{\theta}^{t})} \sum_t \mathcal{L}_t(\boldsymbol{\theta}^{sh},\boldsymbol{\theta}^{t})
\end{align}

\paragraph{Conflicting Gradients}
Let $g_t$ be the gradient of task-specific loss $\mathcal{L}_t$ $w.r.t$ the shared parameters $g_t:=\nabla_{\boldsymbol{\theta}^{sh}} \mathcal{L}_t(\boldsymbol{\theta}^{sh},\boldsymbol{\theta}^{t})$, gradients of task $\mathcal{T}_i$ and $\mathcal{T}_j$ are considered conflicting if $g_i\cdot g_j < 0$. The vanilla update direction of optimizing (\ref{eq:avg_loss}) is usually defined as $G=\sum_{i=1}^T g_i$. There exists two types of conflicting gradients: 
\begin{itemize}
    \item conflicts among the tasks if there exists any two task $\mathcal{T}_i$ and $\mathcal{T}_j$ with $g_i\cdot g_j < 0$
    \item conflicts of the final update direction with the tasks if any task $\mathcal{T}_i$ satisfied that $G\cdot g_i < 0$
\end{itemize}
Since $g_i$  denotes the steepest decreasing direction of task-specific loss $\mathcal{L}_i$ of task $\mathcal{T}_i$ only, conflicts among the tasks are more pervasive especially when the tasks are negatively correlated, leading to conflicts between $G$ and some of the individual tasks. %with decreasing performance of these tasks when updating along $G$. 
As a result, updating $\boldsymbol{\theta}^{sh}$ along the direction of $G$ will decrease the performance of tasks conflicting with $G$.
%The negative effect of conflicting gradients has been a major problem in MTL researches, 
Varies methods have been developed to alleviate such conflicts through different approaches. Some MOO methods focus only on solving conflicts of $G$ with all tasks which are directly responsible for task performance, whereas projection-based methods study conflicts among the tasks since these are the source of all conflicts and most negative effects in MTL.
\paragraph{Pareto stationary points and optimals}
A solution $(\boldsymbol{\theta}^{sh},\boldsymbol{\theta}^{t})$ dominates another $(\boldsymbol{\bar{\theta}}^{sh},\boldsymbol{\bar{\theta}}^{t})$ if $\mathcal{L}_t(\boldsymbol{\theta}^{sh},\boldsymbol{\theta}^{t}) \leq \mathcal{L}_t(\boldsymbol{\bar{\theta}}^{sh},\boldsymbol{\bar{\theta}}^{ t})$ for all $\mathcal{T}_t$ and $\mathcal{L}_t(\boldsymbol{\theta}^{sh},\boldsymbol{\theta}^{t}) < \mathcal{L}_t(\boldsymbol{\bar{\theta}}^{sh},\boldsymbol{\bar{\theta}}^{ t})$ holds for at least one $\mathcal{T}_t$. A solution $\boldsymbol{\theta}^{*}$ is called pareto optimal if no solution dominates $\boldsymbol{\theta}^{*}$. A solution $(\boldsymbol{\theta}^{sh},\boldsymbol{\theta}^{t})$ is called pareto stationary if there exists $\boldsymbol{\alpha} \in \mathbb{R}^T$ such that $\alpha_i \geq 0$, $\sum_{i=1}^T \alpha_i=1$ and $\sum_{i=1}^T \alpha_i g_i = \textbf{0}$. All pareto optimals are pareto stationary, the reverse holds when $\mathcal{L}_t$ is convex for all $\mathcal{T}_t$ \citep{Converge1,Converge2}.
